Provably Secure Disambiguating Neural Linguistic Steganography

Recent research in provably secure neural linguistic steganography has overlooked a crucial aspect: the sender must detokenize stegotexts to avoid raising suspicion from the eavesdropper. The segmentation ambiguity problem, which arises when using language models based on subwords, leads to occasional decoding failures in all neural language steganography implementations based on these models. Current solutions to this issue involve altering the probability distribution of candidate words, rendering them incompatible with provably secure steganography. We propose a novel secure disambiguation method named SyncPool, which effectively addresses the segmentation ambiguity problem. We group all tokens with prefix relationships in the candidate pool before the steganographic embedding algorithm runs to eliminate uncertainty among ambiguous tokens. To enable the receiver to synchronize the sampling process of the sender, a shared cryptographically-secure pseudorandom number generator (CSPRNG) is deployed to select a token from the ambiguity pool. SyncPool does not change the size of the candidate pool or the distribution of tokens and thus is applicable to provably secure language steganography methods. We provide theoretical proofs and experimentally demonstrate the applicability of our solution to various languages and models, showing its potential to significantly improve the reliability and security of neural linguistic steganography systems.

==> 3proposedmethod_old.tex <==
% \begin{figure*}[!t]
%     \centering
%     \includegraphics[width=\textwidth]{figs/flow.pdf}
%     \caption{Our proposed disambiguating method.}
%     \label{fig_flow}
% \end{figure*}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth]{figs/flow2.png}
    \caption{The provably secure disambiguating linguistic steganography consists of the existing provably secure steganography method and our proposed distribution-preserving disambiguation method. We group the original probability distribution by prefix relationships, use the existing provably secure steganography method, e.g. Discop, to embed the message on the grouped distribution, and perform synchronized random sampling from the ambiguous pools using a shared random number between the sender and receiver to ensure unique message extraction. The probability distribution corresponding to the sampled tokens remains unchanged before and after implementing ambiguity elimination.}
    \label{fig_flow}
\end{figure*}
% 无歧义的可证安全隐写方法由现成的可证安全隐写方法和我们提出的不改变分布的消除歧义方法组成。我们将原始概率分布按前缀关系进行合并分组，使用现有的可证安全隐写方法在分组后的分布上进行消息嵌入，在使用发送方与接收方共享的随机数从歧义池中进行可同步的随机采样，保证消息的唯一提取。
% 在实施歧义消除前后，可采样token对应的概率分布不变。

\section{Proposed Method}

As analyzed above, previous attempts at disambiguate introduced damage to the original probability distribution while removing the potentially ambiguous tokens. An adversary can easily get a non-negligible advantage in distinguishing the cover distributions and the stego distributions. % 如上所述，先前试图消除歧义的尝试在移除潜在歧义标记时对原始概率分布造成了损害。攻击者可以轻易获得在区分覆盖分布和隐写分布方面的显著优势。
The ideal method must satisfy the following criteria: (1) the disambiguating algorithm should not alter the model's original probability distribution, all tokens in the candidate pool predicted by the language model should be retained, and each token should maintain its original probability; (2) the disambiguating algorithm should be easily transferable to any generative linguistic steganographic method based on auto-regressive models without being specialized for a specific embedding and extraction algorithm. % 理想的方法必须满足：消除歧义算法不改变模型的原始概率分布，语言模型预测得到的所有的候选池中的token都应该被保留，每一个token都应该保持其原有的概率。
To address this problem, in this section, we present a disambiguating approach based on \textit{group sampling}, which aims to achieve synchronization between the sender and receiver for correctly extracting the message by merging tokens that may cause ambiguity.
% 通过将可能引起歧义的tokens合并，达到发收双方同步以正确提取消息的目的。

Our \textbf{key insight} is that we merge candidate tokens into groups based on whether they are susceptible to segmentation ambiguity, and employing different sampling strategies for suscepted groups. % 我们根据候选标记是否容易受到分段模糊性的影响进行分组，并对受影响的组采用不同的采样策略。
Specifically, the sender firstly searches within the candidate pool to examine if there are tokens whose mapping words are the prefixes of other tokens.
If found, it indicates that the receiver may encounter ambiguity when extracting the message. % 如果存在，说明接收方在提取消息时可能会产生歧义。
At this point, we identify all tokens in the candidate pool that share the same prefix, grouping them together as the ambiguous pools. 
After that, the steganographic embedding algorithm performs message-driven sampling on the merged distribution. % 这之后，隐写嵌入算法在归并后的分布上根据消息进行隐写采样。
If the sampling result is an ambiguous pool, a pre-shared random number between the sender and receiver is consumed to randomly sample from the ambiguous pool. % 如果采样结果是一个歧义池，则消耗一个发送方与接收方事先共享的随机数在歧义候选池中随机采样。
In this method, the number of sampleable tokens and the probability of each token remains unchanged compared to the original probability distribution. % 在这一过程中，每个可采样的token的概率与原始概率分布相比没有被改变。
The disambiguating steganography embedding process is shown in \autoref{fig_flow}.


For the receiver, before attempting to extract the secret message from a token, they first check the ambiguous pool associated with the token to be extracted. If the token does not carry segmentation ambiguity risks, the receiver proceeds to extract the secret message using the steganographic extraction algorithm as usual. % 对于接收方，在尝试对token进行隐写消息提取前，先检查与待提取token相关的歧义候选池，如果歧义候选池中只有待提取的token一个元素，说明该token没有分割歧义风险，正常使用隐写提取算法提取出秘密消息；
However, if there is more than one element in the ambiguous pool, the receiver checks whether the current tokenized token was sampled using the shared random number. If it was, it indicates that the token received by the receiver is synchronized with the token selected by the sender. If not, token list correction is required. % 如果不止一个元素，则在歧义候选池中检查当前token是否是由共享随机数驱动采样得到的，如果是，说明接收方得到的token已经与发送方的选择的token同步了，如果不是，则需要进行token列表的纠错。
The corresponding message needs to be extracted from the merged probability interval corresponding to the entire ambiguous pool. % 对应的消息需要以整个歧义池对应的概率区间进行提取。

\subsection{Candidate Pool with Original Distribution}

During normal generation, the language model can predict the probability distribution of the next token $x_t$ given previous context $x_{<t}$ in the whole vocabulary $\Sigma$,
\begin{equation}
    \text{Pr}\left[x_t|x_{<t}\right] = \left[p_1, p_2, \dots, p_{\left|\Sigma\right|}\right],\nonumber
\end{equation}
where $p_1$ through $p_{\left|\Sigma\right|}$ respectively represent the probabilities of tokens $c_1$ through $c_{\left|\Sigma\right|}$ in the vocabulary, holding that $\sum_{i=1}^{\left|\Sigma\right|}p_i=1$.

Then, the model needs to sample a token from the distribution mentioned above and add it to the generated sequence. There are primarily two sampling methods: \textit{greedy sampling} and \textit{random sampling}. In most cases, users of the generative language model desire the model's output to exhibit variability and creativity while maintaining a level of controlled randomness. Therefore, to ensure that the model's output meets specific requirements or matches desired styles, three crucial parameters are introduced during the random sampling process. They are temperature, top-$p$, and top-$k$. 
% 注意到，模型需要从上述分布中采样一个token加入生成序列，采样方法主要有两种：贪心采样和随机采样。而用户一般情况下希望模型的输出拥有一些变化性和创造性，但又不愿意这种随机性不受控制。因此，为了使模型的输出满足特定要求或匹配所需风格，三个至关重要的参数在随机采样过程中被引入，他们分别是：温度，top-p和top-k。

The temperature influences the shape of the probability distribution that the model calculates for the next token rather than limiting the token selection. 
Top-$p$, a.k.a. nucleus sampling~\cite{holtzman2019curious}, allows for dynamic control of the number of tokens considered, leading to different levels of diversity in the generated text, while top-$k$ provides a controlled randomness by considering a fixed number of top probable tokens, 
Three of them could change the distributions or candidate pools of $x_t$. 
% As observed, GPT-2~\cite{radford2019language} has 50,257 candidate tokens, while Baichuan2~\cite{baichuan2023baichuan2} has as many as 125,696 candidate tokens.
It is common to use these parameters to control random sampling in the normal sampling process of innocent users.
Therefore, in provably secure steganography, there should be no restrictions on the use of these parameters. Additionally, reducing the size of the candidate pool using the top-$p$ and top-$k$ methods significantly reduces the computational overhead of both random sampling and generative steganography. 
% As observed, for GPT-2~\cite{radford2019language} with 50,257 candidate tokens, the top-$p$ truncation ($p\neq1.00$) eliminates a substantial number of candidate tokens, resulting in negligible additional time.
% For these large language models, whether or not steganography is performed, truncating the distribution with appropriate means is necessary.

Therefore, in this paper, we define the \textbf{original distribution} as the probability after applying these probability processing methods, and the \textbf{original candidate pool} as the remaining available tokens after the top-$k$ or top-$p$ stage, which does not contradict the behavioral security pursued by steganography.
% 因此，在本文中我们定义原始载体分布为经过这些概率处理方法之后的概率，原始候选池为经过top-p或top-k阶段之后剩余的可选token。这与隐写追求的行为安全并不矛盾。

\begin{definition}
    The original distribution of the language model before steganography refers to the probability distribution composed of the remaining tokens after probability processing. Let $V$ denote the remaining \textbf{candidate pool}, $V=\left[c_1, c_2, \dots, c_{\left|V\right|}\right]$, $\left|V\right|\leq\left|\Sigma\right|$. The \textbf{original distribution} is $P_c=\left[p_1, p_2, \dots, p_{\left|V\right|}\right]$, holding that $\sum_{i=1}^{\left|V\right|}p_i\leq1$. % 模型的原始分布指经过概率处理后剩余的token组成的概率分布。
\end{definition}

Provable secure steganography requires that steganography does not alter the original distribution predicted by the model. Therefore, the candidate pool and distribution after disambiguation must also remain consistent with $V$ and $P_c$. % 可证安全隐写要求隐写不改变模型预测的原始分布，则适用于可证安全隐写的消除歧义方法处理之后的候选池和分布亦需与V和P_c保持一致。


\subsection{Ambiguous Pool}

Like the existing disambiguation approaches, our approach also needs to identify all potential candidate words that could cause ambiguity. % 就像其他已有的消除歧义方法一样，我们的方法也需要找到所有可能引起歧义的候选词。
The \textbf{prefix relationship} between candidate words is a necessary but not sufficient condition for segmentation ambiguity to occur. % 候选词之间的前缀关系是发生分割歧义的必要不充分条件。

\begin{definition}
    In the candidate pool, tokens exhibit \textbf{prefix relationships}, meaning that for a specified token $\ct$ in the candidate pool, its mapping subword either serves as a prefix for other tokens' or there exist other tokens whose mapping words are prefixes of this token's. That is $\exists c_i \in \Vt, c_i \neq \ct$, such that $\textsc{prefix}\left(\ct, c_i\right) = 1$ or $\textsc{prefix}(c_i, \ct) = 1$. % 候选池中token存在前缀关系，指对于一个在候选池中的指定token，其是其他token的前缀或存在其他token是该token的前缀。
\end{definition}

Here $\textsc{prefix}\left(c_i, c_j\right)$ donates a prefix relationship:
\begin{equation}
    \textsc{prefix}\left(c_i, c_j\right) = 
    \begin{cases}
        1, & c_i \text{ is a prefix of } c_j , \\
        0, & \text{otherwise} .
    \end{cases} \nonumber
\end{equation}

\begin{figure}[t]
    \centering
    \subfloat[$D$ /wo prefix relationships]{\includegraphics[width=0.4\columnwidth]{figs/examplecase1.png}}%
    \label{fig_first_case_1}
    \hfil
    \subfloat[$BB$ /w prefix relationships]{\includegraphics[width=0.4\columnwidth]{figs/examplecase2.png}}%
    \label{fig_first_case_2}
    \caption{Different cases about prefix relationship.}
    \label{fig_prefix}
\end{figure}

\autoref{fig_prefix} illustrates two scenarios: one where the selected token has no prefix relationship with other tokens in the candidate pool, and another where it does. Given a candidate pool of the top-$8$, $V=[AA,B,CCC,D,BB,BBD,C,BDD]$. When the selected token is $D$, there is no prefix relationship; when it is $BB$, two other tokens, $B$ and $BBD$, have a prefix relationship with it. % 图中给出了选定token与候选池中的其他token没有前缀关系和有前缀关系的两种情况。给定候选池是一个top-8的情况，V=[AA,B,CCC,D,BB,BBD,C,BDD]. 当给定token是D时，不存在前缀关系；当给定token是BB是，有其他两个token B和BBD与其存在前缀关系。
The previous disambiguation algorithms removed certain tokens to ensure that there were no prefix relationships in the candidate pool. However, the approach we implemented in this paper is to establish a new group for tokens that have prefix relationships. We name it the \textbf{ambiguity pool}. % 之前的消除歧义算法的做法是去除某些token来确保候选池中不存在前缀关系。而我们在本文中实现的方法是为这些存在前缀关系的token建立一个新的分组。我们将其命名为歧义池。
In this paper, establishing an ambiguity pool that can synchronize between the sender and the receiver is the key to our disambiguating algorithm. % 建立一个能在发送方与接收方之间同步的歧义池是本文方法的关键。

% We find that simply conducting a search for prefix relationships with a given token is not feasible. % 简单的对一个给定token进行前缀关系的查找是行不通的。
% The specific reasons will be provided after the completion of the method description. % 具体原因我们将在方法流程描述完毕之后给出。
% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{figs/ambiguioupool.png}
%     \caption{Example for building an ambiguous pool when given a chosen token $BB$ in \autoref{fig_prefix}'s candidate pool.}
%     \label{fig_ambiguouspool}
% \end{figure}


\begin{algorithm}[t]
\caption{$\textsc{Ambiguity}\left(\ct, \Vt, P_\ct\right)$: Construct an Ambiguity Pool of Given Token $\ct$ on Candidate Pool $\Vt$}\label{algo_ambiguouspool}

\SetAlgoLined

\KwIn{Candidate Pool $\Vt=\left[c_1, c_2, \dots, c_{\left|V\right|}\right]$; Candidate Distribution $P_\ct=\left[p_1, p_2, \dots, p_{\left|V\right|}\right]$; Given token $\ct$;} 
\KwOut{Ambiguity Pool $V_{amb}^{(t)}=\left[c_{amb,1}, c_{amb,2}, \dots, c_{amb,\left|V_{amb}\right|}\right]$; Ambiguity Distribution $P_{amb}^{(t)}=\left[p_{amb,1}, p_{amb,2}, \dots, p_{amb,\left|V_{amb}\right|}\right]$;}

\tcc{initialization}
$V_{amb}^{(t)}\leftarrow\emptyset$\text{,\ }$P_{amb}^{(t)}\leftarrow P_\ct$\;

\tcc{find the shortest prefix token}
$\ct_{short}\leftarrow\ct$\;
\For{$c_i$ in $\Vt$}{
    \If{$\textsc{Prefix}\left(c_i, \ct\right)$ and $\textsc{Len}\left(c_i\right)<\textsc{Len}\left(\ct_{short}\right)$}{
        $\ct_{short}\leftarrow c_i$\;
    }
}

\tcc{add all ambiguous tokens}
\For{$c_j$ in $\Vt$}{
    \eIf{$\textsc{Prefix}\left(\ct_{short}, c_j\right)$}{
        $V_{amb}^{(t)}\textsc{.append}(c_j)$\;
    }{
        $p_{amb,j}\leftarrow0$
    }
}

\tcc{normalization}
$P_{amb}^{(t)}\leftarrow\frac{P_{amb}^{(t)}}{\sum_{i=1}^{\left|V^{(t)}\right|}p_{amb,i}}$
% \tcp*{normalization}

\textbf{return}
\end{algorithm}


Using the distribution constructed in \autoref{fig_prefix} as an example, if the selected token is $BB$, we first find the shortest token $B$ that has a prefix relationship with $BB$. Then, we search for prefix relationships in the top-$8$ candidate pool for $B$, adding $B$, $BB$, $BBD$, and $BDD$ to the ambiguity pool, $V_{amb}=[B,BB,BBD,BDD]$. % 用图4中构造的分布举例，如果选定的token为BB，先找到与其有前缀关系的最短token B，然后在top-8候选池中对B进行前缀关系的查找，将B、BB、BBD、BDD加入歧义池。
The process of constructing the ambiguity pool in this example is illustrated in \autoref{fig_ambiguouspool}. % 这个例子中构建歧义池的过程如图所示。
For comparison, if we only search for tokens with prefix relationships with $BB$, the constructed ambiguity pool would lack $BDD$ because $BB$ is not a prefix of $BDD$.% 作为对比，如果只查找与BB有前缀关系的token，构造的歧义池中会缺少BDD，因为BB不是BDD的前缀。

The specific algorithm for constructing the ambiguity pool is shown in \autoref{algo_ambiguouspool}. % 构建歧义池的具体算法如算法所示。
Formally, given a chosen token $\ct$ for the $t$-th step, we first need to find the shortest token $c_{short}^{(t)}$ that has a prefix relationship with it. Then, based on this shortest token, we add all tokens in the candidate pool $\Vt$ that have $\ct$ as a prefix to the ambiguity pool, % 给定一个token，我们需要先找到与其有前缀关系的最短token，然后以这个最短token为基础，将候选池中所有以其为前缀的token都加入歧义池。
We then establish a new distribution, denoted as $P_{amb}^{(t)}$, for these elements in $V_{amb}^{(t)}$ such that the probability of each token remains consistent with the original probability distribution, and then normalize the distribution. % 我们为$V_{amb}^{(t)}$中的这些元素建立一个新的分布，记为P，每个token的概率保持与原始概率分布中一致，然后对分布进行归一化。
The final ambiguity pool and its corresponding probabilities,
\begin{equation}
    V_{amb}^{(t)}, P_{amb}^{(t)}\leftarrow\textsc{Ambiguity}\left(\ct, \Vt, P_c^{(t)}\right). \nonumber
\end{equation}


\subsection{Synchronous Random Sampling}

With the ambiguity pool, the sender and receiver can synchronize tokens prone to segmentation ambiguity before and after detokenization and tokenization using a pre-shared random number. % 有了歧义池，发送方和接收方可以使用一个事先共享的随机数实现detokenize和tokenize前后可能发生分割歧义的token的同步。
We name this stage \textbf{synchronous random sampling}. 

Formally, let $V_{amb}^{(t)}$ be the ambiguity pool of $\ct$ for step $t$, and $P_{amb}^{(t)}$ be its corresponding probability distribution for synchronous random sampling. 
We generate a random number shared between the sender and receiver using a synchronous PRNG, donated as ${PRNG}_{sync}$. As long as the sender and receiver share an initial seed, they can obtain a series of synchronized pseudo-random numbers $\mathbf{r}=\left\{r^{(0)}, r^{(1)}, \dots\right\}$, which follows the uniform distribution on $\left[0,1\right)$, i.e., $r^{(t)}\sim U\left[0,1\right)$. % 我们采取的方法是，生成一个发送方与接收方共享的随机数，该随机数可以通过一个PRNG生成，只要发送方与接收方共享一个初始化种子，就能得到一个同步的伪随机数序列，每个随机数都服从0-1均匀分布。
At each time step $t$, each token in the ambiguous pool $V_{amb}^{(t)}$ is allocated to the left-closed, right-open interval $\left[0,1\right)$ according to $P_{amb}^{(t)}$. Then, we consume a pseudo-random number $r^{(t)}$ and select the token corresponding to the interval to which $r^{(t)}$, donated as the synchronous token $c_{sync}$,
\begin{equation}
    c_{sync}^{(t)} \leftarrow \textsc{SyncSample}\left(P_{amb}^{(t)}, r^{(t)}\right). \nonumber
\end{equation}
As long as both the sender and the receiver have access to the same ambiguity pool, they can utilize the shared random number to determine a token known to the other party. % 只要发送方和接收方可以得到一个相同的歧义池，就可以利用他们双方共享的随机数从中确定一个对方可知的token。

We know that segmentation ambiguity refers to the situation where the stegotext is incorrectly tokenized by the receiver into tokens different from those generated by the sender. This occurs only when the sender's token and the receiver's token exhibit prefix relationship. % 我们知道，分割歧义是指隐写文本被接收方错误地tokenize成了与发送方生成的不同的token，这只会发生在发送端token与接受端token拥有相同的前缀的时候。
The purpose of synchronous sampling is to inform the receiver which token the sender has chosen from the ambiguity pool. % 同步采样的作用是使接收方获知发送方在歧义池中选择的是哪一个token，
However, this does not directly eliminate segmentation ambiguity because we have not altered the size or distribution of the candidate pool, and those tokens capable of triggering segmentation ambiguity will still be sampled according to their original probabilities. % 但这事实上并不能直接消除分割歧义，因为我们没有改变候选池的大小和分布，能够触发分割歧义的那些token仍会以其原本的概率被采样到。
Therefore, it is necessary to design a token reconstruction mechanism for the receiver that can work in conjunction with synchronous sampling. 
% 因此，必须为接收方设计可以配合同步采样的token重建机制。


% Suppose the receiver is extracting a message from the $t$-th token in hand. All previous $t-1$ tokens have undergone correct steganographic extraction without segmentation ambiguity. Let the token generated by the sender be denoted as $\ct_{send}$ and the token tokenized from the receiver be denoted as $\ct_{recv}$.
% % 假设接收方正在对他手中的第t个token进行消息提取，之前的全部t-1个token都没有发生分割歧义，已经正确完成了隐写提取。记发送端token为$\ct_{send}$，接受端token为$\ct_{recv}$。

% In cases of ambiguity, there are only two possible scenarios: % 在歧义发生时，只可能有两种情况：
% \paragraph{$\ct_{send}$ is the prefix of $\ct_{recv}$}
% An intuitive example is when ``\_any'' and ``thing'' generated by the sender are tokenized by the receiver as ``\_anything'', where $\ct_{send}=\text{``\_any''}$, $c^{(t+1)}_{send}=\text{``thing''}$, and $\ct_{recv}=\text{``\_anything''}$.
% % 一个直观的例子是，发送方生成的“any”和“thing”被接收方标记成了“anything”。

% \paragraph{$\ct_{recv}$ is the prefix of $\ct_{send}$}
% Similar examples include when $\ct_{send}=\text{``\_anything''}$, while $\ct_{recv}=\text{``\_any''}$, and $c^{(t+1)}_{recv}=\text{``thing''}$.



















Next, we will describe the complete process of provably secure steganography after introducing our proposed disambiguation algorithm, including steganographic embedding and steganographic extraction.
% 接下来我们会描述引入我们所提出的消歧算法后的可证安全隐写的完整流程，包括隐写嵌入和隐写提取。

\subsection{Embedding}

\begin{algorithm}[t]
\SetAlgoLined
\caption{$\textsc{Embedding}$}\label{algo_embedding}
\KwIn{Context $C$, $\text{PRNG}_{steg}$, $\text{PRNG}_{sync}$, Language Model $\mathcal{M}$, Tokenizer $\mathcal{T}$, Seed $K$, Message $\mathbf{m}$}%输入参数
\KwOut{Stegotext $S$}%输出

\begin{minipage}[t]{0.3\columnwidth}
$x\leftarrow\emptyset$\;
\end{minipage}
\hfill
\begin{minipage}[t]{0.5\columnwidth}
\raggedleft
\texttt{// Stego Tokens}
\end{minipage}

$\text{PRNG.}\textsc{SetSeed}\left(K\right)$\;
$t\leftarrow1$

\While{\textbf{not} the end of $\mathbf{m}$}{
    \begin{minipage}[t]{0.5\columnwidth}
    $\Vt, P_c^{(t)}\leftarrow \mathcal{M}\left(C\right)$\;
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.3\columnwidth}
    \raggedleft
    \texttt{// predict}
    \end{minipage}
    $\ct\leftarrow\textsc{Encode}_{P_\ct}\left(\text{PRNG}_{steg}(K)^{(t)}, \mathbf{m}\right)$\;

    \eIf{\textbf{not} ambiguous}{
	$x_t \leftarrow \ct$\;
        $\mathbf{m} \leftarrow \mathbf{m}\left[\textsc{EmbedNum}\left(\ct,P_\ct\right):\right]$\;
    }{
	$V_{amb}^{(t)}, P_{amb}^{(t)}\leftarrow\textsc{Ambiguity}\left(\ct, \Vt, P_c^{(t)}\right)$\;
        $c_{sync}^{(t)} \leftarrow \textsc{SyncSample}\left(P_{amb}^{(t)}, \text{PRNG}_{sync}(K)^{(t)}\right)$\;
        $x_t \leftarrow c_{sync}^{(t)}$\;

        % $\mathbf{m} \leftarrow \mathbf{m}\left[\textsc{EmbedNum}\left(V_{amb}^{(t)},P_\ct\right):\right]$\;
    }
    $x\textsc{.append}(x_t)$\;
    $C\leftarrow C\parallel x_t$\;
    $t\leftarrow t+1$\;
}
$S\leftarrow \mathcal{T}.\textsc{Decode}\left(x\right)$\;
\textbf{return}
\end{algorithm}


The main loop of provably secure steganographic message embedding process with our proposed disambiguating algorithm is shown in \autoref{algo_embedding}.
At the $t$-th step of generation, the steganography embedding algorithm provides a token to be output based on the original distribution $P_\ct$, a random number provided by the ${PRNG}_{steg}$ giving the Key $K$, and the message bit sequence $\mathbf{m}$, % 具体而言，在发送方的生成阶段，发送方先实施隐写嵌入算法。在第t步生成，隐写嵌入算法会根据模型分布、PRNG给出的随机数、消息比特序列，给定一个待输出的token。
\begin{equation}
    \ct\leftarrow\textsc{Encode}_{P_\ct}\left({PRNG}_{steg}(K)^{(t)}, \mathbf{m}\right). \nonumber
\end{equation}

If there are no other tokens in the candidate pool $\Vt$ whose mapping words have a prefix relationship with the given token $\ct$, it can be retained and added into the stego sequence, i.e., $x_t\leftarrow\ct$, and the steganographic message embedding and generation process can proceed normally. % 如果$V_{amb}^{(t)}$中只有一个元素，即在候选池中没有其他与给定token有前缀关系的token，可以保留ct，正常完成一次隐写消息嵌入和生成。

However, if $\ct$ is an ambiguous token, which means $V_{amb}^{(t)}$ corresponding to $\ct$ contains more than one element, indicating a potential error in message extraction by the receiver. At this point, we employ the synchronous sampling method proposed in the previous section for token synchronization. % 但如果$V_{amb}^{(t)}$中不止一个元素，说明接收方在提取时可能会发生错误，需要进行token的同步。
The result of steganographic embedding is rolled back, and the synchronized ambiguous token $\ct$ will be added to the stego token sequence.
% 隐写采样的结果被回退，而将同步有歧义token被加入载密token序列。
% Accordingly, since all ambiguous tokens are grouped, the steganographic embedding rate will also be altered. % 相应的，由于所有有歧义的token被我们分为一组，隐写嵌入率也会被改变。
Specifically, in the event of ambiguity, the steganographic embedding process does not select a specific token, but rather selects a group of tokens that may cause ambiguity. % 具体来说，在发生歧义的情况下，隐写嵌入过程不是选择了某一个具体的token，而是选择了一个可能发生歧义的token组成的分组。
% The information that can be embedded is determined by the probability of this group. % 可以被嵌入的信息由这个分组的概率决定。
The message is not embedded in this process. % 在这个过程中不嵌入消息。

Finally, the sender needs to decode the stego tokens using a tokenizer into stegotext before transmission.
% 在隐写嵌入完成后，发送方需要将stego tokens使用tokenizer解码成stegotext再进行传输。

\subsection{Extraction}

\begin{algorithm}[t]
\SetAlgoLined
\caption{$\textsc{Extraction}$}\label{algo_extraction}
\KwIn{Stegotext $S$, Context $C$, $\text{PRNG}_{steg}$, $\text{PRNG}_{sync}$, Language Model $\mathcal{M}$, Tokenizer $\mathcal{T}$, Seed $K$}%输入参数
\KwOut{Message $\mathbf{m}$}%输出
$\mathbf{m}\leftarrow\text{``\ ''}$\;
$x\leftarrow\emptyset$\;
$\text{PRNG.}\textsc{SetSeed}\left(K\right)$\;
$t\leftarrow1$\;

\While{\textbf{not} the end of $S$}{
    \begin{minipage}[t]{0.5\columnwidth}
    $\Vt, P_c^{(t)}\leftarrow \mathcal{M}\left(C\right)$\;
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.3\columnwidth}
    \raggedleft
    \texttt{// predict}
    \end{minipage}

    $\ct\leftarrow\textsc{PrefixToken}\left(S,\Vt\right)$\;
    % let $\ct$ be the first token in $\Vt$ being a prefix of $S$\;
    \eIf{\textbf{not} ambiguous}{
	$x_t \leftarrow \ct$\;
        $\mathbf{m}_t\leftarrow\textsc{Decode}_{P_\ct}\left(\text{PRNG}_{steg}(K)^{(t)}, x_t\right)$\;
    }{
	$V_{amb}^{(t)}, P_{amb}^{(t)}\leftarrow\textsc{Ambiguity}\left(\ct, \Vt, P_c^{(t)}\right)$\;
        $c_{sync}^{(t)} \leftarrow \textsc{SyncSample}\left(P_{amb}^{(t)}, \text{PRNG}_{sync}(K)^{(t)}\right)$\;
        $x_t \leftarrow c_{sync}^{(t)}$\;
        
        
        % $\mathbf{m}_t\leftarrow\textsc{Decode}_{P_\ct}\left(\text{PRNG}_{steg}(K)^{(t)}, V_{amb}^{(t)}\right)$\;
    }

    $x\textsc{.append}(x_t)$\;
    % $x\leftarrow x\parallel x_t$\;
    $C\leftarrow C\parallel x_t$\;
    
    $S\leftarrow S\left[\textsc{Len}\left(\mathcal{T}.\textsc{Decode}\left(x_t\right)\right):\right]$\;
    $\mathbf{m}\leftarrow \mathbf{m}\parallel \mathbf{m}_t$\;

    $t\leftarrow t+1$\;
    
}
\textbf{return}
\end{algorithm}

The main loop of provably secure steganographic message extraction process with our proposed disambiguating algorithm is shown in \autoref{algo_extraction}. 
During extraction, unlike the previous ambiguity-unaware provably secure steganography, the receiver needs to first abandon using the off-the-shelf tokenizer to tokenize the stegotext directly.% 在提取时，与之前的歧义不敏感的可证安全隐写流程不同的是，接收方需要首先放弃使用现成的tokenizer直接对stegotext进行标记化。
At each time step of auto-regressive generation process, the receiver selects a token $\ct$ from the candidate pool $\Vt$, while $\ct$ is a prefix of the remaining part of the detokenized stegotext $S$. % 在自回归生成过程的每个时间步中，接收方从候选池 $\Vt$ 中选择一个标记 $\ct$，而 $\ct$ 是解标记化后隐写文本 $S$ 剩余部分的前缀。
The receiver checks whether the selected token may induce ambiguity, in other words, whether there are some other words that have a prefix relationship with $\ct$. If so, the receiver also construct an ambiguity pool $\Vt_{amb}$ of $\ct$ and employs the same synchronous sampling as the sender to synchronize the tokens. % 接收方检查选择出的文本是否可能诱发歧义，若是，接收方也采用与发送方相同的同步采样，来完成token的同步。


\subsection{Proof of Security}

In this scenario, the next token is obtained through two rounds of sampling. The first is the message-driven steganographic embedding algorithm's sampling from the candidate pool, and the second is the random sampling driven by a shared random number in the ambiguity pool.
The first round of sampling uses a provably secure steganographic algorithm, which maintains the original distribution. If a non-ambiguous token without common prefixes is sampled, the sampling ends.
If a token that may cause ambiguity is sampled, a second round of sampling is conducted. The sampling pool for the second round is the ambiguity pool of the token sampled in the first round. At this point, the result of the first round of sampling is essentially an equivalent token composed of all the tokens in this sampling pool together, and the second round selects a specific one from this equivalent token. This is actually a process of conditional sampling from the distribution.
% 下面分析安全性。
% 在这种情况下，下一个token是经过两次采样才得到的。第一次是消息驱动的隐写嵌入算法在候选池中的采样，第二次是在歧义池中由共享随机数驱动的随机采样.
% 首先，第一次采样使用的是可证安全的隐写算法，算法保持了原始分布。若采样到的是不存在共同前缀的非歧义token，采样结束。
% 若采样到的是可能发生歧义的token，再进行第二次采样。第二次采样的采样池是第一次采样token的歧义池。这时，第一次采样的结果实际上是由这个采样池中的所有token共同组成的一个等价token，第二次才是从这个等价token中选择一个具体的。这实际上是一次分布条件采样的过程。



% \begin{align}
%     P\left[x_t\right] 
%         &= P\left[\ct|\text{$\ct$ not ambiguous}\right] + P\left[\ct|\text{$\ct$ ambiguous}\right]\\
%         &= 
% \end{align}

==> old_exptable.tex <==

\begin{table*}[!t]
\centering
\caption{Quantitative comparison with the previous disambiguating methods on Discop using LLaMA2 and English context.}\label{tab_exp_en}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{@{}cc|ccccccccc@{}}
\toprule
\multicolumn{2}{c|}{Method} & $k$ & Ave PPL & Ave KLD $\downarrow$ & Max KLD $\downarrow$ & \begin{tabular}[c]{@{}c@{}}Capacity $\uparrow$\\ (bits/token)\end{tabular} & Utilization $\uparrow$ & \begin{tabular}[c]{@{}c@{}}Total Time $\downarrow$\\ (seconds)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Ave Time $\downarrow$\\ (seconds)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Total Error $\downarrow$\\ (\%)\end{tabular} \\ \midrule
\multicolumn{2}{c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Discop\end{tabular}}} & 16 & 3.27 & 0 & 0 & 1.30 & 0.84 & 480.10 & 3.68E-02 & 1.81 \\
\multicolumn{2}{c|}{} & 32 & 3.50 & 0 & 0 & 1.44 & 0.85 & 479.57 & 3.32E-02 & 2.80 \\
\multicolumn{2}{c|}{} & 64 & 3.88 & 0 & 0 & 1.58 & 0.85 & 480.84 & 3.04E-02 & 2.74 \\
\multicolumn{2}{c|}{} & 128 & 4.20 & 0 & 0 & 1.70 & 0.87 & 484.49 & 2.84E-02 & 2.50 \\
\multicolumn{2}{c|}{} & 256 & 4.55 & 0 & 0 & 1.81 & 0.88 & 487.83 & 2.69E-02 & 2.67 \\ \midrule
\multicolumn{1}{c|}{\multirow{15}{*}{\begin{tabular}[c]{@{}c@{}}Discop +\end{tabular}}} & \multirow{5}{*}{Basic} & 16 & 12.13 & 30.25 & 98.63 & 1.58 & 0.86 & 477.83 & 3.02E-02 & 0 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 32 & 18.75 & 37.34 & 98.64 & 1.93 & 0.86 & 483.34 & 2.51E-02 & 0 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 64 & 29.67 & 44.02 & 98.63 & 2.38 & 0.86 & 488.30 & 2.05E-02 & 0 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 128 & 42.26 & 49.10 & 98.63 & 2.80 & 0.85 & 508.60 & 1.82E-02 & 0 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 256 & 63.73 & 53.17 & 98.63 & 3.18 & 0.87 & 580.46 & 1.83E-02 & 0 \\ \cmidrule(l){2-11} 
\multicolumn{1}{c|}{} & \multirow{5}{*}{MWIS} & 16 & 2.64 & 2.72 & 64.64 & 1.01 & 0.77 & 489.93 & 4.87E-02 & 0 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 32 & 2.83 & 2.94 & 71.56 & 1.12 & 0.76 & 500.53 & 4.47E-02 & 0 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 64 & 3.04 & 3.41 & 72.96 & 1.22 & 0.77 & 525.99 & 4.31E-02 & 0 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 128 & 3.22 & 3.58 & 68.56 & 1.29 & 0.76 & 986.66 & 7.66E-02 & 0 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 256 & 3.52 & 3.79 & 72.34 & 1.38 & 0.77 & 3765.48 & 2.73E-01 & 0 \\ \cmidrule(l){2-11} 
\multicolumn{1}{c|}{} & \multirow{5}{*}{SyncPool} & 16 & 3.19 & \textbf{0} & \textbf{0} & 1.00 & 0.66 & 484.14 & 4.84E-02 & 0 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 32 & 3.74 & \textbf{0} & \textbf{0} & 1.03 & 0.59 & 487.56 & 4.75E-02 & 0 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 64 & 3.88 & \textbf{0} & \textbf{0} & 0.85 & 0.46 & 488.99 & 5.74E-02 & 0 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 128 & 4.50 & \textbf{0} & \textbf{0} & 0.63 & 0.31 & 488.00 & 7.73E-02 & 0 \\
\multicolumn{1}{c|}{} & \multicolumn{1}{c|}{} & 256 & 4.96 & \textbf{0} & \textbf{0} & 0.39 & 0.18 & 491.68 & 1.27E-01 & 0 \\ 
\bottomrule
\end{tabular}
}
\end{table*}

\begin{table*}[!t]
\centering
\caption{Quantitative comparison with the previous disambiguating methods on Discop using Baichuan2 and Chinese context.}\label{tab_exp}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{@{}cc|ccccccccc@{}}
\toprule
\multicolumn{2}{c|}{Method} & $k$ & Ave PPL & Ave KLD $\downarrow$ & Max KLD $\downarrow$ & \begin{tabular}[c]{@{}c@{}}Capacity $\uparrow$\\ (bits/token)\end{tabular} & Utilization $\uparrow$ & \begin{tabular}[c]{@{}c@{}}Total Time $\downarrow$\\ (seconds)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Ave Time $\downarrow$\\ (seconds)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Total Error $\downarrow$\\ (\%)\end{tabular} \\ \midrule
\multicolumn{2}{c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Discop\end{tabular}}} & 16 & 8.16 & 0 & 0 & 2.03 & 0.88 & 693.96 & 3.42E-02 & 1.73 \\
\multicolumn{2}{c|}{} & 32 & 10.97 & 0 & 0 & 2.56 & 0.90 & 691.17 & 2.70E-02 & 4.36 \\
\multicolumn{2}{c|}{} & 64 & 13.96 & 0 & 0 & 2.98 & 0.91 & 690.69 & 2.31E-02 & 5.36 \\
\multicolumn{2}{c|}{} & 128 & 20.12 & 0 & 0 & 3.60 & 0.93 & 692.19 & 1.92E-02 & 5.32 \\
\multicolumn{2}{c|}{} & 256 & 26.17 & 0 & 0 & 3.99 & 0.94 & 1000.93 & 2.51E-02 & 6.30 \\ \midrule
\multicolumn{1}{c|}{\multirow{15}{*}{\begin{tabular}[c]{@{}c@{}}Discop +\end{tabular}}} & \multirow{5}{*}{Basic} & 16 & 12.96 & 25.54 & 98.63 & 1.97 & 0.87 & 841.25 & 4.28E-02 & 0 \\
\multicolumn{1}{l|}{} &  & 32 & 20.22 & 30.34 & 98.63 & 2.48 & 0.86 & 867.03 & 3.50E-02 & 0 \\
\multicolumn{1}{l|}{} &  & 64 & 34.87 & 36.12 & 98.63 & 3.03 & 0.89 & 906.46 & 2.99E-02 & 0 \\
\multicolumn{1}{l|}{} &  & 128 & 45.63 & 38.36 & 98.59 & 3.32 & 0.87 & 950.55 & 2.86E-02 & 0 \\
\multicolumn{1}{l|}{} &  & 256 & 67.07 & 40.91 & 98.62 & 3.68 & 0.87 & 1056.15 & 2.87E-02 & 0 \\ \cmidrule(l){2-11} 
\multicolumn{1}{c|}{} & \multirow{5}{*}{MWIS} & 16 & 6.63 & 6.89 & 62.76 & 1.60 & 0.75 & 705.43 & 4.42E-02 & 0 \\
\multicolumn{1}{l|}{} &  & 32 & 8.71 & 8.20 & 61.90 & 2.05 & 0.77 & 712.56 & 3.48E-02 & 0 \\
\multicolumn{1}{l|}{} &  & 64 & 12.15 & 9.87 & 64.48 & 2.55 & 0.78 & 723.59 & 2.84E-02 & 0 \\
\multicolumn{1}{l|}{} &  & 128 & 14.82 & 10.85 & 65.60 & 2.86 & 0.78 & 826.53 & 2.89E-02 & 0 \\
\multicolumn{1}{l|}{} &  & 256 & 19.50 & 11.92 & 67.10 & 3.23 & 0.78 & 2131.85 & 6.60E-02 & 0 \\ \cmidrule(l){2-11} 
\multicolumn{1}{c|}{} & \multirow{5}{*}{SyncPool} & 16 & 7.49 & \textbf{0} & \textbf{0} & 1.57 & 0.72 & 695.04 & 4.42E-02 & 0 \\
\multicolumn{1}{l|}{} &  & 32 & 10.93 & \textbf{0} & \textbf{0} & 2.08 & 0.74 & 692.46 & 3.33E-02 & 0 \\
\multicolumn{1}{l|}{} &  & 64 & 14.40 & \textbf{0} & \textbf{0} & 2.46 & 0.74 & 693.70 & 2.82E-02 & 0 \\
\multicolumn{1}{l|}{} &  & 128 & 19.16 & \textbf{0} & \textbf{0} & 2.78 & 0.73 & 695.98 & 2.50E-02 & 0 \\
\multicolumn{1}{l|}{} &  & 256 & 23.57 & \textbf{0} & \textbf{0} & 3.05 & 0.73 & 700.90 & 2.30E-02 & 0 \\ 
% \midrule
% \multicolumn{2}{c|}{\multirow{5}{*}{Random   Sampling}} & 16 & 19.61 & 0 & 0 & N/A & N/A & 694.13 & N/A & N/A \\
% \multicolumn{2}{c|}{} & 32 & 26.77 & 0 & 0 & N/A & N/A & 690.98 & N/A & N/A \\
% \multicolumn{2}{c|}{} & 64 & 32.52 & 0 & 0 & N/A & N/A & 689.86 & N/A & N/A \\
% \multicolumn{2}{c|}{} & 128 & 42.19 & 0 & 0 & N/A & N/A & 906.42 & N/A & N/A \\
% \multicolumn{2}{c|}{} & 256 & 53.12 & 0 & 0 & N/A & N/A & 867.31 & N/A & N/A \\ 
\bottomrule
\end{tabular}
}
\end{table*}
